ALMA 1.3 mm Survey of Lensed Submillimeter Galaxies (SMGs) Selected by Herschel: Discovery of Spatially Extended SMGs and Implications

We present an ALMA 1.3 mm (Band 6) continuum survey of lensed submillimeter galaxies (SMGs) at $z=1.0\sim3.2$ with an angular resolution of $\sim0.2$". These galaxies were uncovered by the Herschel Lensing Survey (HLS), and feature exceptionally bright far-infrared continuum emission ($S_\mathrm{peak} \gtrsim 90$ mJy) owing to their lensing magnification. We detect 29 sources in 20 fields of massive galaxy clusters with ALMA. Using both the Spitzer/IRAC (3.6/4.5 $\mathrm{\mu m}$) and ALMA data, we have successfully modeled the surface brightness profiles of 26 sources in the rest-frame near- and far-infrared. Similar to previous studies, we find the median dust-to-stellar continuum size ratio to be small ($R_\mathrm{e,dust}/R_\mathrm{e,star} = 0.38\pm0.14$) for the observed SMGs, indicating that star formation is centrally concentrated. This is, however, not the case for two spatially extended main-sequence SMGs with a low surface brightness at 1.3 mm ($\lesssim 0.1$ mJy arcsec$^{-2}$), in which the star formation is distributed over the entire galaxy ($R_\mathrm{e,dust}/R_\mathrm{e,star}>1$). As a whole, our SMG sample shows a tight anti-correlation between ($R_\mathrm{e,dust}/R_\mathrm{e,star}$) and far-infrared surface brightness ($\Sigma_\mathrm{IR}$) over a factor of $\simeq$ 1000 in $\Sigma_\mathrm{IR}$. This indicates that SMGs with less vigorous star formation (i.e., lower $\Sigma_\mathrm{IR}$) lack central starburst and are likely to retain a broader spatial distribution of star formation over the whole galaxies (i.e., larger $R_\mathrm{e,dust}/R_\mathrm{e,star}$). The same trend can be reproduced with cosmological simulations as a result of central starburst and potentially subsequent "inside-out" quenching, which likely accounts for the emergence of compact quiescent galaxies at $z\sim2$.

==> 98c_difflens.tex <==
% All of our discussions above are based on the assumption that differential lensing effect is not applied.
% However, due to the finite source size, the lensing magnification exerted to different regions in the same SMG will exhibit a spatial variation.
% Therefore, in this subsection we will briefly discuss the affect of differential lensing to our main results.

%% stop here

As pointed out by \citet{hezaveh12}, for a two-component lensed source model (i.e., a compact core plus an extended halo or disk), the compact component can be magnified with a much larger factor than the diffuse one when the overall magnification factor is high ($\gtrsim 10$).
Based on published cluster mass models of MACS1115 and MACS0553 \citep{oguri10,zitrin15,ebeling17}, we derive a median magnification factor of $\sim 5$ for HLS1115 and HLS0553-A/B/C.
Similar magnification can also be estimated from a comparison of median lensed $R_\mathrm{e,star}$ and $M_\mathrm{star}$ with mass--radius relation of early-type galaxies at similar redshift \citep{vdw14}.
Therefore, a significant number of SMGs in this study are significantly magnified (especially those extended and low-$\Sigma_\mathrm{IR}$ ones), meaning that such a bias of magnification factor could affect the observed relation seen in Figure~\ref{fig:08_main} and thus Figure~\ref{fig:10_quench}.

The anti-correlation seen in the left panel of Figure~\ref{fig:10_quench} should remain valid when the effect of differential magnification is considered.
For example, if the dust component is more extended than the stellar one (i.e.,  $R_\mathrm{e,dust}/R_\mathrm{e,star} > 1$), then the magnification of the stellar component should be larger than that of the dust component according to \citet{hezaveh12}, and thus the intrinsic $R_\mathrm{e,dust}/R_\mathrm{e,star}$ should be even larger.
Conversely, $R_\mathrm{e,dust}/R_\mathrm{e,star} < 1$ sources will have smaller intrinsic dust-to-stellar size ratio, and thus the linear relation in Figure~\ref{fig:08_main} (left panel) can have an even steeper slope if differential lensing effect is corrected. 
However, we also note that in the cluster lensing cases, the extended component is more likely to cross the caustics and get strongly amplified because of a larger angular area.
In this regard, the distribution of observed source size ratio is stretched in the left panel of Figure~\ref{fig:08_main}, and thus the intrinsic slope might be more gradual.

Although it still remains difficult to determine the effect of differential magnification on overall SED shapes (e.g., dust temperature and IRAC color), the anti-correlation between $R_\mathrm{e,dust} / R_\mathrm{e,star}$ (and thus $\mathrm{sSFR}_\mathrm{t}/\mathrm{sSFR}_\mathrm{c}$) and central sSFR remains valid.  
Therefore, our interpretation in Section~\ref{sss:05a_iiquench} is not an artifact of differential magnification.


%  we examine the effect of differential lensing in individual lens systems by modeling each source as a compact core embedded in an extended diffuse halo. Considering the ratio of magnifications in these two components, we find that at high overall magnifications, the compact component is amplified by a much larger factor than the diffuse component, but at intermediate magnifications (∼10) the probability of a larger magnification for the extended region is higher. Lens models determined from multi-frequency resolved imaging data are crucial to correct for this effect.
